On the use of automatically generated synthetic image datasets for benchmarking face recognition

The availability of large-scale face datasets has been key in the progress of face recognition. However, due to licensing issues or copyright infringement, some datasets are not available anymore (e.g. MS-Celeb-1M). Recent advances in Generative Adversarial Networks (GANs), to synthesize realistic face images, provide a pathway to replace real datasets by synthetic datasets, both to train and benchmark face recognition (FR) systems. The work presented in this paper provides a study on benchmarking FR systems using a synthetic dataset. First, we introduce the proposed methodology to generate a synthetic dataset, without the need for human intervention, by exploiting the latent structure of a StyleGAN2 model with multiple controlled factors of variation. Then, we confirm that (i) the generated synthetic identities are not data subjects from the GAN's training dataset, which is verified on a synthetic dataset with 10K+ identities; (ii) benchmarking results on the synthetic dataset are a good substitution, often providing error rates and system ranking similar to the benchmarking on the real dataset.

==> Makefile <==
TEXFILE=main.tex
PDFFILE=$(TEXFILE:%.tex=%.pdf)

%.pdf: %.tex
	pdflatex $(@:%.pdf=%.tex); \
	bibtex $(@:%.pdf=%); \
	pdflatex $(@:%.pdf=%.tex); \
	pdflatex $(@:%.pdf=%.tex)

all: $(PDFFILE)

.PHONY: clean

clean:
	@rm -vf *.log *.lot *.lof *.loa *.toc *.idx *.inc *.ilg *.ind *.bbl *.blg
	@rm -vf *.aux *.glo *.dvi *.ps *.pdf *.out *.brf


==> sections/rebuttal.tex <==

\section*{Rebuttal}

\vspace{-0.3cm}
\subsection*{Reviewers 1 \& 2}
\vspace{-0.3cm}
We thank the reviewers for their remarks on possible extensions of this work to better assess the preservation of identity when performing the face editing. The suggestion from reviewer 1 to measure facial landmarks to study the preservation of face shape is particularly interesting as it can potentially be done in an automated manner. Both this experiment, as well as a perceptual study with human raters, will be considered in future work.
\vspace{-1cm}
\subsection*{Reviewer 3}
\vspace{-0.3cm}
We thank the reviewer for his questions and provide hereafter some additional information on the evoked technical details.

\textbf{Architecture and performance of the networks}
Because we are using the same architectures for benchmarking the real and synthetic datasets, and are more interested in the performance comparison that in the raw error rates, we considered the \emph{direct} inclusion of certain technical architecture details to be redundant since they are available through the cited references for each model. Moreover, all our face recognition models will be accessible at the time of source code release. We still include here some additional details for the consideration of the reviewers.

\vspace{-0.3cm}
\textbf{Inception-ResNet models} The Inception-ResNet models used for the ICT constraint and for the benchmark experiments originate from \cite{pereira_heterogeneous_2019}\footnote{Numbered citations refer to the bibliography in the submitted article.}. They are reusing an open source implementation\footnote{https://github.com/davidsandberg/facenet} of a FaceNet model, and are trained using a mixture of cross-entropy and center loss\footnote{https://ydwen.github.io/papers/WenECCV16.pdf} for the loss. The ICT model in particular is \emph{trained} on MS-Celeb; our use of the term ``pretrained" was maybe unnecessarily confusing. To compute the ICT, we indeed first synthesize face images associated to the candidate latents, then forward those images through the FR model to obtain the face embeddings of interest.

\vspace{-0.3cm}
\textbf{ArcFace model} We indeed use the InsightFace implementation\footnote{https://github.com/deepinsight/insightface}, and more specifically the ResNet-100 variant. Regarding the performance of our variant retrained on VGGFace2, we emphasize that the smaller size of the VGGFace2 dataset is not necessarily incompatible with an increased performance. In \cite{cao_vggface2_2018}, which originally introduces VGGFace2, they compare the performance of various models trained respectively on MS-Celeb and VGGFace2. They showcase a generally better performance when training on VGGFace2 (despite it being smaller than MS-Celeb), which they explain by a better quality of the dataset labels.

\textbf{Se-Se-ROC} The study of the Se-Se-ROC and of the worst Se-Se impostor pairs might indeed provide more insight on possible demographic differentials of the FR model. However, this investigation is more related to the field of bias and fairness in face recognition, and is out of the scope of this work.

\textbf{Scaling of the intra-subject variation} The choice of using the average (instead of maximal) distance of image projections to the separation hyperplane as the scaling reference aims to avoid a \emph{single} projected latent to fully define the scaling. It also puts a greater emphasis on ensuring a better preservation of identity, albeit with the possible effect of synthesizing weaker variations. Finally, it produced the qualitatively better visual results; the exploration of alternative choices will be considered for future work.

\textbf{Relation between ICT value and generation runtime}
We present in figure \ref{fig:measuredruntime} an experiment of runtime measurement with an ICT value of 0.2.  We observe a runtime growth that is lesser than exponential but greater than polynomial in the number of identities. A fit of the form $t(x) = A\exp\left({Cx^p}\right)$, with $t$ the runtime and $x$ the number of identities, predicts a runtime of around 8000 days to reach 11k identities, which is of course unpractical. Note that this extrapolated value must still be taken with much caution as the expression of the fit is not theoretically grounded. Anyway, in comparison, it takes only around 1.5 hours to generate 11k identities with an ICT value of 0.1. Note that higher ICT values can still be used for generating smaller datasets, however the higher the ICT, the more expensive it becomes to scale the number of identities.

\begin{figure}[ht]
	\centering
	\includegraphics[width=0.7\linewidth]{figures/measured_runtime}
	\caption{Measured runtime for generation of $\sim3000
		$ identities with ICT 0.2 on a GTX 1080 Ti. The fit takes the expression $t = 2.7\cdot 10^{-5} \exp \left(1.84\cdot x^{0.27} \right)$ with $t$ the runtime in hours and $x$ the number of identities.}
	\label{fig:measuredruntime}
	\vspace{-0.3cm}
\end{figure}


